HREF: Human Response-Guided Evaluation of Instruction Following in Language Models

Evaluating the capability of Large Language Models (LLMs) in following instructions has heavily relied on a powerful LLM as the judge, introducing unresolved biases that deviate the judgments from human judges. In this work, we reevaluate various choices for automatic evaluation on a wide range of instruction-following tasks. We experiment with methods that leverage human-written responses and observe that they enhance the reliability of automatic evaluations across a wide range of tasks, resulting in up to a 3.2% improvement in agreement with human judges. We also discovered that human-written responses offer an orthogonal perspective to model-generated responses in following instructions and should be used as an additional context when comparing model responses. Based on these observations, we develop a new evaluation benchmark, Human Response-Guided Evaluation of Instruction Following (HREF), comprising 4,258 samples across 11 task categories with a composite evaluation setup, employing a composite evaluation setup that selects the most reliable method for each category. In addition to providing reliable evaluation, HREF emphasizes individual task performance and is free from contamination. Finally, we study the impact of key design choices in HREF, including the size of the evaluation set, the judge model, the baseline model, and the prompt template. We host a live leaderboard that evaluates LLMs on the private evaluation set of HREF.

==> sections/103-method.tex <==
\paragraph{Goal} Given an instruction, \ourmethod\ aims to select the better response between two model, known as pairwise comparison~\citep{zheng2023judging}. With \ours, \ourmethod\ is additionally provided with a human-written response as reference. 

\ourmethod\ contains three evaluation methods as below, see the formal defination of them in Appendix~\ref{app:formulation}.

\begin{enumerate}
    \item \textbf{\ourllm} uses LLM-as-a-Judge~\citep{zheng2023judging}, where it directly prompts a powerful LLM to judge the a pair responses from two models. See Appendix~\ref{app:llm-template} for the prompt template we use.
    \item \textbf{\ourllmwhf} is similar to \ourllm\ except that we embed the human reference into the prompt and ask the judge LLM to refer to it when making the judgment. See Appendix~\ref{app:llm-template} for the prompt template we use. 
    \item \textbf{\ourrb} computes the cosine similarity of RoBERTa text embeddings~\citep{DBLP:journals/corr/abs-1907-11692} between a model response and the human reference as the score for that response, and select the response with higher score.
\end{enumerate}

For each of the category, we select one of these methods that performs the best in our human agreement analysis (See Section~\ref{sec:agreement-evaluation}). See Table~\ref{tab:evaluators} for the specific evaluation method selections. 

Note that we allow the methods to judge ``tie" between the two model responses.

\paragraph{Implementation Details.} We use Llama-3.1-Instruct-70B~\citep{dubey2024llama} as the judge LLM and RoBERTa-Large for obtaining text embeddings. See Section~\ref{sec:discussion} for more explanation of such choices.






==> sections/104-agreement.tex <==
\newcommand{\oursb}{65.3}
\newcommand{\oursoq}{60.5}
\newcommand{\ourscq}{73.0}
\newcommand{\ourse}{75.6}
\newcommand{\oursg}{70.3}
\newcommand{\oursr}{75.4}
\newcommand{\ourss}{68.0}
\newcommand{\oursc}{68.1}
\newcommand{\oursf}{71.5}
\newcommand{\oursm}{66.0}
\newcommand{\oursro}{73.8}
\newcommand{\ourso}{69.4}

\newcommand{\hub}{62.6}
\newcommand{\huoq}{59.5}
\newcommand{\hucq}{71.9}
\newcommand{\hue}{73.8}
\newcommand{\hug}{66.3}
\newcommand{\hur}{69.9}
\newcommand{\hus}{63.4}
\newcommand{\huc}{69.8}
\newcommand{\huf}{71.0}
\newcommand{\hum}{62.8}
\newcommand{\huro}{74.3}
\newcommand{\huo}{67.0}

\newcommand{\lgb}{50.1}
\newcommand{\lgoq}{33.3}
\newcommand{\lgcq}{28.3}
\newcommand{\lge}{38.1}
\newcommand{\lgg}{49.1}
\newcommand{\lgr}{52.6}
\newcommand{\lgs}{40.5}
\newcommand{\lgc}{43.3}
\newcommand{\lgf}{39.0}
\newcommand{\lgm}{54.8}
\newcommand{\lgro}{45.8}
\newcommand{\lgo}{43.1}

\newcommand{\shb}{43.8}
\newcommand{\shoq}{61.6}
\newcommand{\shcq}{65.6}
\newcommand{\she}{57.6}
\newcommand{\shg}{49.0}
\newcommand{\shr}{45.5}
\newcommand{\shs}{56.6}
\newcommand{\shc}{52.9}
\newcommand{\shf}{57.8}
\newcommand{\shm}{42.8}
\newcommand{\shro}{53.5}
\newcommand{\sho}{53.2}

\newcommand{\rab}{46.3}
\newcommand{\raoq}{49.5}
\newcommand{\racq}{41.1}
\newcommand{\rae}{47.7}
\newcommand{\rag}{54.9}
\newcommand{\rar}{47.3}
\newcommand{\ras}{50.1}
\newcommand{\rac}{50.0}
\newcommand{\raf}{45.3}
\newcommand{\ram}{44.8}
\newcommand{\raro}{50.0}
\newcommand{\rao}{48.2}

\newcommand{\gtb}{60.0}
\newcommand{\gtoq}{49.1}
\newcommand{\gtcq}{54.8}
\newcommand{\gte}{67.8}
\newcommand{\gtg}{66.6}
\newcommand{\gtr}{68.6}
\newcommand{\gts}{53.3}
\newcommand{\gtc}{52.1}
\newcommand{\gtf}{56.3}
\newcommand{\gtm}{60.0}
\newcommand{\gtro}{69.0}
\newcommand{\gto}{59.4}

\newcommand{\gtwmb}{58.9}
\newcommand{\gtwmoq}{54.1}
\newcommand{\gtwmcq}{50.2}
\newcommand{\gtwme}{71.3}
\newcommand{\gtwmg}{64.4}
\newcommand{\gtwmr}{70.9}
\newcommand{\gtwms}{52.5}
\newcommand{\gtwmc}{57.5}
\newcommand{\gtwmf}{70.5}
\newcommand{\gtwmm}{62.5}
\newcommand{\gtwmro}{55.3}
\newcommand{\gtwmo}{60.2}

\newcommand{\gtwb}{60.1}
\newcommand{\gtwoq}{53.3}
\newcommand{\gtwcq}{63.1}
\newcommand{\gtwe}{69.3}
\newcommand{\gtwg}{65.6}
\newcommand{\gtwr}{70.1}
\newcommand{\gtws}{59.0}
\newcommand{\gtwc}{57.5}
\newcommand{\gtwf}{59.8}
\newcommand{\gtwm}{64.8}
\newcommand{\gtwro}{72.3}
\newcommand{\gtwo}{62.6}

\newcommand{\gttb}{65.5}
\newcommand{\gttoq}{57.1}
\newcommand{\gttcq}{63.6}
\newcommand{\gtte}{72.5}
\newcommand{\gttg}{63.9}
\newcommand{\gttr}{72.5}
\newcommand{\gtts}{61.9}
\newcommand{\gttc}{62.5}
\newcommand{\gttf}{61.5}
\newcommand{\gttm}{64.5}
\newcommand{\gttro}{69.8}
\newcommand{\gtto}{64.8}

\newcommand{\gttwmb}{67.1}
\newcommand{\gttwmoq}{62.1}
\newcommand{\gttwmcq}{65.0}
\newcommand{\gttwme}{71.7}
\newcommand{\gttwmg}{64.4}
\newcommand{\gttwmr}{74.0}
\newcommand{\gttwms}{62.9}
\newcommand{\gttwmc}{66.2}
\newcommand{\gttwmf}{69.3}
\newcommand{\gttwmm}{62.8}
\newcommand{\gttwmro}{57.5}
\newcommand{\gttwmo}{65.9}

\newcommand{\gttwb}{65.5}
\newcommand{\gttwoq}{58.8}
\newcommand{\gttwcq}{67.8}
\newcommand{\gttwe}{75.6}
\newcommand{\gttwg}{63.1}
\newcommand{\gttwr}{72.5}
\newcommand{\gttws}{64.4}
\newcommand{\gttwc}{68.1}
\newcommand{\gttwf}{64.3}
\newcommand{\gttwm}{62.5}
\newcommand{\gttwro}{70.5}
\newcommand{\gttwo}{66.4}

\newcommand{\lsb}{59.9}
\newcommand{\lsoq}{55.5}
\newcommand{\lscq}{49.5}
\newcommand{\lse}{64.8}
\newcommand{\lsg}{56.1}
\newcommand{\lsr}{64.3}
\newcommand{\lss}{57.5}
\newcommand{\lsc}{57.8}
\newcommand{\lsf}{63.8}
\newcommand{\lsm}{56.3}
\newcommand{\lsro}{64.5}
\newcommand{\lso}{58.7}

\newcommand{\lswmb}{60.0}
\newcommand{\lswmoq}{51.4}
\newcommand{\lswmcq}{45.9}
\newcommand{\lswme}{63.5}
\newcommand{\lswmg}{51.8}
\newcommand{\lswmr}{63.8}
\newcommand{\lswms}{54.9}
\newcommand{\lswmc}{54.1}
\newcommand{\lswmf}{61.5}
\newcommand{\lswmm}{51.3}
\newcommand{\lswmro}{70.0}
\newcommand{\lswmo}{56.5}

\newcommand{\lswb}{56.5}
\newcommand{\lswoq}{53.1}
\newcommand{\lswcq}{47.2}
\newcommand{\lswe}{65.8}
\newcommand{\lswg}{53.1}
\newcommand{\lswr}{63.0}
\newcommand{\lsws}{54.3}
\newcommand{\lswc}{55.5}
\newcommand{\lswf}{68.5}
\newcommand{\lswm}{52.5}
\newcommand{\lswro}{63.8}
\newcommand{\lswo}{56.8}

\newcommand{\lmb}{65.3}
\newcommand{\lmoq}{58.5}
\newcommand{\lmcq}{64.8}
\newcommand{\lme}{69.7}
\newcommand{\lmg}{64.1}
\newcommand{\lmr}{73.4}
\newcommand{\lms}{68.0}
\newcommand{\lmc}{66.0}
\newcommand{\lmf}{69.0}
\newcommand{\lmm}{63.5}
\newcommand{\lmro}{66.8}
\newcommand{\lmo}{66.2}

\newcommand{\lmwmb}{65.0}
\newcommand{\lmwmoq}{55.4}
\newcommand{\lmwmcq}{69.2}
\newcommand{\lmwme}{75.6}
\newcommand{\lmwmg}{67.8}
\newcommand{\lmwmr}{76.3}
\newcommand{\lmwms}{66.1}
\newcommand{\lmwmc}{68.9}
\newcommand{\lmwmf}{70.5}
\newcommand{\lmwmm}{68.3}
\newcommand{\lmwmro}{65.0}
\newcommand{\lmwmo}{67.7}

\newcommand{\lmwb}{62.5}
\newcommand{\lmwoq}{55.3}
\newcommand{\lmwcq}{73.0}
\newcommand{\lmwe}{75.6}
\newcommand{\lmwg}{70.3}
\newcommand{\lmwr}{75.4}
\newcommand{\lmws}{66.9}
\newcommand{\lmwc}{68.1}
\newcommand{\lmwf}{64.0}
\newcommand{\lmwm}{66.0}
\newcommand{\lmwro}{73.8}
\newcommand{\lmwo}{67.9}

\newcommand{\bemb}{64.1}
\newcommand{\bemoq}{66.5}
\newcommand{\bemcq}{64.8}
\newcommand{\beme}{76.4}
\newcommand{\bemg}{68.5}
\newcommand{\bemr}{67.6}
\newcommand{\bems}{60.1}
\newcommand{\bemc}{64.6}
\newcommand{\bemf}{71.3}
\newcommand{\bemm}{66.0}
\newcommand{\bemro}{65.8}
\newcommand{\bemo}{66.4}

\newcommand{\beb}{48.4}
\newcommand{\beoq}{60.5}
\newcommand{\becq}{68.8}
\newcommand{\bee}{69.9}
\newcommand{\beg}{64.1}
\newcommand{\ber}{64.8}
\newcommand{\bes}{61.0}
\newcommand{\bec}{61.9}
\newcommand{\bef}{71.5}
\newcommand{\bem}{55.5}
\newcommand{\bero}{70.0}
\newcommand{\beo}{62.5}

\newcommand{\romb}{61.3}
\newcommand{\romoq}{66.8}
\newcommand{\romcq}{67.7}
\newcommand{\rome}{73.4}
\newcommand{\romg}{63.3}
\newcommand{\romr}{69.0}
\newcommand{\roms}{57.5}
\newcommand{\romc}{59.0}
\newcommand{\romf}{67.3}
\newcommand{\romm}{67.5}
\newcommand{\romro}{64.0}
\newcommand{\romo}{64.7}

\newcommand{\rob}{52.4}
\newcommand{\rooq}{57.3}
\newcommand{\rocq}{70.3}
\newcommand{\roe}{65.0}
\newcommand{\rog}{58.0}
\newcommand{\ror}{70.4}
\newcommand{\ros}{55.0}
\newcommand{\roc}{50.0}
\newcommand{\rof}{70.3}
\newcommand{\rom}{61.5}
\newcommand{\roro}{61.0}
\newcommand{\roo}{60.3}

\newcommand{\ppb}{47.9}
\newcommand{\ppoq}{51.5}
\newcommand{\ppcq}{57.1}
\newcommand{\ppe}{51.8}
\newcommand{\ppg}{48.8}
\newcommand{\ppr}{42.8}
\newcommand{\pps}{52.9}
\newcommand{\ppc}{42.1}
\newcommand{\ppf}{54.9}
\newcommand{\ppm}{52.8}
\newcommand{\ppro}{59.7}
\newcommand{\ppo}{50.3}

\begin{figure}
\centering \footnotesize
\resizebox{0.8\columnwidth}{!}{\includegraphics[trim={0.5cm 0.5cm 0.5cm 0.5cm},clip]{figures/fig-length_distribution.pdf}}
\caption{
\textbf{The distribution of length difference between sampled model responses and the base line model responses}. The distribution is symmetrical.
}\label{fig:length-distribution}
\end{figure}

To demonstrate the alignment between \ours's judgments and human preference, we construct a dataset that contains instruction and responses from a variety of models, collect human annotations on the pairwise preference between response pairs, and compare the agreement of \ours\ with the collected human labels, along with other baselines.

\subsection{Dataset Construction}
In this subsection, we construct a dataset composed by instructions, responses from models and human, along with human labeled preference, which we perform the agreement analysis with.

\subsubsection{Instructions and Responses Collection}\label{subsec:human-agreement-instruction-collection}
Here, we describe the construction and composition detail of the instructions and responses in our human agreement set described in Section~\ref{sec:dataset}.
\paragraph{Instruction Set.} Because the instructions in our validation set has an extremely skewed distribution across different categories, and the prompts are scarce in some specific categories like Extraction, we choose to combine part of the developement set data with the data from the train split of No Robots. We additionally sample data in the three science categories that are not present the No Robots. We ended up with 438 instructions where all 11 categories are reasonably represented (See Figure~\ref{fig:dataset-distribution}).

\paragraph{Model Pool.} In order to ensure the diversity of the responses, we build a model pool with 32 LLMs with sizes from 7B to over 100B and more than 10 different model families to compare against the baseline model. See the full list in Appendix~\ref{app:human-set-model-pool}.


\paragraph{Response Sampling.} For each instruction, we sample responses from 4 distinct models to pair with the baseline model. To ensure that we are not creating any implicit bias about the response lengths (e.x., the longer response is always better), we separate all model response for each instruction into two groups based on whether a response is longer or shorter than the baseline model response. We then randomly sample 2 response from each of the 2 groups. To ensure the quality of the response and avoid looping repetitions in generation, we use a decoding temperature of 1.0 for all the models. Figure~\ref{fig:length-distribution} shows the resulting distribution of the length difference between sampled model responses and baseline model responses. The symmetrical distribution shows that both the shorter and the longer responses are fairly sampled. 

\subsubsection{Human Annotation Collection.}\label{subsec:annotation-collection}
We describe how we collect 4 human preference annotations for each pair of model responses in this section.   

\paragraph{Annotator Selection.} To control the quality of the annotations, we limit our annotator choices to English-native speakers only from the U.S., the U.K., and Canada, who must have  Bachelor's degrees or above from Prolific~\citep{Prolific_2014}. We also require the annotators to have have a approval rate over 99\% in the studies that they have participated in the past. We launch a qualification study as where a participant needs to correctly annotation at least 9 out of 10 straightforwardly distinguishable model response pairs to pass. We assign the qualification task to 50 participants, and recruit 16 of them as our final group of annotators. We set the hourly salary to be \$16 / hour.

\paragraph{Guideline.}
We adopt and modify the guideline for human annotator from \citet{alpaca_eval}, where a checklist of judging aspects and two examples are provided to the annotators. In response of the circumstance where two responses are similar, we include the option of "tie" beyond the binary options. See the full guideline in Appendix~\ref{app:human-guideline}. 

\paragraph{Interface.} 
We modify the website for collecting human annotations based on \citet{miranda2024hybrid}. We redirect the annotations from Prolific to this website and ask them to carefully read the instructions. During the annotation process, besides the instruction and the two pairs of model responses are available on the right, all the guidelines and a simple preference selection button are available for the annotators on the right. To avoid potential bias in order of the responses, we randomly swap the two responses.

\paragraph{Statistics.}
We successfully collect 7,008 annotations on 1,752 model pairs. The annotators spend around 180s with a standard deviation of 79s on each annotations on average with a tie rate of 4.9\%.

\subsection{Baseline}\label{subsec:baselines}
To understand the level of agreement with human of \ourmethod, we compare \ourmethod\ against a list of evaluators described as following:

\textbf{Random} randomly select one of the two responses in uniform distribution.

\textbf{Shorter \slash\ Longer} naively always prefer the shorter  \slash\ longer response.

\textbf{Perplexity} calculates and compares the perplexities of the human written reference answer conditioned on the instruction between the two models.

\textbf{Rouge~\citep{lin2004rouge}} calculates a score using the overlap between n-grams of the model response and the human written reference answer, and it then select the response with the higher score. We use Rouge-1 (unigram) in the experiment.

\paragraph{\ourmethod\ variants.} In addition to the simple baseline methods above, we evaluate each unit evaluator in \ourmethod\ individually with four LLM judges, including GPT-4 and GPT-4-Turbo~\citep{achiam2023gpt} that prior benchmarks use.

\begin{table*}[t!]
    \centering  \small
    \setlength{\tabcolsep}{4.5pt}
    \begin{tabular}{p{0.19\linewidth} c c c c c c c c c c c c}
    \toprule
        \multirow{2}{*}{Method} & \multicolumn{8}{c}{General Category} & \multicolumn{3}{c}{Science Category}  & \multirow{2}{*}{All} \\
        \cmidrule(lr){2-9} \cmidrule(lr){10-12} &
         Brn & OQA & CQA & Ext & Gen & Rew & Sum & Cls & FC & MDS & RND  \\
    \midrule
        \textit{Simple Baselines} \\
        Shorter & \shb & \shoq & \shcq & \she & \shg & \shr & \shs & \shc & \shf & \shm & \shro & \sho \\
        Longer & \lgb & \lgoq & \lgcq & \lge & \lgg & \lgr & \lgs & \lgc & \lgf & \lgm & \lgro & \lgo \\
        Random & \rab & \raoq & \racq & \rae & \rag & \rar & \ras & \rac & \raf & \ram & \raro & \rao \\
        Rouge & \rob & \rooq & \rocq & \roe & \rog & \ror & \ros & \roc & \rof & \rom & \roro & \roo \\
        Perplexity & \ppb & \ppoq & \ppcq & \ppe & \ppg & \ppr & \pps & \ppc & \ppf & \ppm & \ppro & \ppo \\
    \midrule
        \multicolumn{8}{l}{\textit{\ourllm}} \\
        GPT4 & \gtb & \gtoq & \gtcq & \gte & \gtg & \gtr & \gts & \gtc & \gtf & \gtm & \gtro & \gto \\
        GPT4-Tb & \gttb & \gttoq & \gttcq & \gtte & \gttg & \gttr & \gtts & \gttc & \gttf & \gttm & \gttro & \gtto \\
        Llama-7B & \lsb & \lsoq & \lscq & \lse & \lsg & \lsr & \lss & \lsc & \lsf & \lsm & \lsro & \lso \\
        \textbf{Llama-70B} & \lmb & \lmoq & \lmcq & \lme & \lmg & \lmr & \lms & \lmc & \lmf & \lmm & \lmro & \lmo \\
    \midrule
        \multicolumn{8}{l}{\textit{\ourllmwhf}} \\
        GPT4 + Ref & \gtwb & \gtwoq & \gtwcq & \gtwe & \gtwg & \gtwr & \gtws & \gtwc & \gtwf & \gtwm & \gtwro & \gtwo \\
        GPT4-Tb + Ref& \gttwb & \gttwoq & \gttwcq & \gttwe & \gttwg & \gttwr & \gttws & \gttwc & \gttwf & \gttwm & \gttwro & \gttwo \\
        Llama-7B + Ref & \lswb & \lswoq & \lswcq & \lswe & \lswg & \lswr & \lsws & \lswc & \lswf & \lswm & \lswro & \lswo \\
        \textbf{Llama-70B }& \lmwb & \lmwoq & \lmwcq & \lmwe & \lmwg & \lmwr & \lmws & \lmwc & \lmwf & \lmwm & \lmwro & \lmwo \\
    \midrule
        \multicolumn{8}{l}{\textit{\ourrb}} \\
        \textbf{RoBERTa-Large} & \beb & \beoq & \becq & \bee & \beg & \ber & \bes & \bec & \bef & \bem & \bero & \beo \\
    \midrule
        \textbf{\ourmethod} & \oursb & \oursoq & \ourscq & \ourse & \oursg & \oursr & \ourss & \oursc & \oursf & \oursm & \oursro & \textbf{\ourso} \\
    \midrule
        Human & \hub & \huoq & \hucq & \hue & \hug & \hur & \hus & \huc & \huf & \hum & \huro & \huo \\
    \bottomrule
    \end{tabular}\vspace{-.1em}
    \caption{
    \textbf{Human Agreement Rates of Different Evaluators on 11 Categories.} All numbers are average LOO agreement rates in \%. Brn $\rightarrow$ Brainstorm; OQA $\rightarrow$ Open QA; CQA $\rightarrow$ Closed QA; Ext $\rightarrow$ Extraction; Gen $\rightarrow$ Generation; Rew $\rightarrow$ Rewriting; Sum $\rightarrow$ Summarization; Cls $\rightarrow$ Classification; FC $\rightarrow$ Fact Checking / Attributed QA; MDS $\rightarrow$ Multi-Document Synthesis; RND $\rightarrow$ Reasoning Over Numerical Data. When calculating Perplexity, we omit some instances in the human agreement datasets where the perplexity are not available with OpenAI models.
 }\label{tab:agreement-results}
\end{table*}

\begin{figure}
\centering \footnotesize
\resizebox{0.8\columnwidth}{!}{\includegraphics[trim={0.5cm 0.5cm 0.5cm 0.5cm},clip]{figures/fig-length_difference.pdf}}
\caption{
\textbf{Length Bias Rate of Different LLM Judges}. It is clear that Llama-3.1-70B Instruct has the least length bias, and such bias is further reduce when using human reference.
}\label{fig:length-difference}
\end{figure}

\subsection{Metrics}
Following \citet{alpaca_eval}, we calculate the \textbf{Leave-One-Out (LOO) agreement rate} for each set of 4 annotations by computing the accuracy of using the evaluator preference prediction \slash\ one of the annotation to predict the mode of the other three and taking the average of this accuracy over the 4 annotations. We report the human agreement rate as the average of LOO agreement rate over the all response pairs. See Appendix~\ref{app:loo} for the detailed algorithm. 


\subsection{Results}\label{subsec:results}
Table~\ref{tab:agreement-results} shows the results of the human agreement analysis. 

\paragraph{Agreement varies across task categories. } For open-ended task categories including Brainstorm, Open QA, and Multi-Document Synthesis, agreements across all evaluators are lower, indicating that human possess divergent standards for judging LLMs diverges, and they weights various dimension of such open-ended responses differently. On the other hands, categories that tends to have easily verifiable answers, including Close QA, Extraction, Classification, and Reasoning Over Numerical Data, appears to have higher agreements. Note that although Rewrite contains many open-ended instructions, a large portion of the instructions are verifiable as they ask for specific tone or format of the response. These findings highlight the importance to evaluate LLMs on specific task categories.

\paragraph{Human written reference improves LLM-as-a-Judge. } Across models including GPT-4, GPT-4-Turbo, and Llama-3.1-70B-Instruct, we frequently see improvements in human agreements when embedding the human written responses into the prompts and using them as reference answers. 
 The results suggest that human written reference can help improve the judgment both explicitly and implicitly, despite that the reference writers and the annotators are two different group of people. They can explicitly be checked against for correctness when dealing with verifiable instructions from Close QA, Extraction, Classification, and Reasoning Over Numerical Data, with a increment of 3.7\% in agreement rate on average with Llama-3.1-70B-Instruct. They also encapsulate implicit aspects in human preference when dealing with Generation, with a 4.2\% increment in agreement rate with Llama-3.1-70B-Instruct. We see an agreement drop when using the reference only with Llama-3.1-7B-Instruct. It is likely because LLMs have to reach a certain capability threshold so that they understand how to properly utilize the reference. See the comparison of human written reference against model-generated reference in Section~\ref{subsec:model-generated}. See examples of how human written reference facilitate judge models in Appendix~\ref{app:ref-help}.

 \paragraph{Prompting judge model and measuring similarity with human reference are complementary.} For Open QA and Fact Checking / Attributed QA with Llama-3.1-70B-Instruct, we see that using human reference as part of the prompt for LLM-as-a-Judge causes a drop in performance. However, using Bert-score brings an performance improvement in contrasts. This shows that using a different evaluator for different task category can allow us to better leverage human reference. Thus, we select either LLM with human reference or Bert-score for each task category in \ours\ based on this human agreement analysis. For categories, including Brainstorm and Summarization, we do not use human reference as they hurt performance. Overall, \ourmethod\ is able to outperform human annotator's innner agreement rate. See the full evaluator list that we choose for each category in Table~\ref{tab:evaluators}.




\begin{table*}[t!]
    \centering  \small
    % \setlength{\tabcolsep}{4.5pt}
    \begin{tabular}{ll}
    \toprule
         Category & Evaluation Method \\
    \midrule
        Brainstorm & \ourllm \\
        Open QA & \ourrb \\
        Closed QA & \ourllmwhf \\
        Extraction & \ourllmwhf \\
        Generation & \ourllmwhf \\
        Rewriting & \ourllmwhf \\
        Summarization & \ourllm \\
        Classification & \ourllmwhf \\
        Fact Checking / Attributed QA &  \ourrb \\
        Multi-Document Synthesis & \ourllmwhf \\
        Reasoning Over Numerical Data & \ourllmwhf \\
    \bottomrule
    \end{tabular}\vspace{-.1em}
    \caption{
    \textbf{List of the evaluation method \ourmethod\ uses for each category.} We use Llama-3.1-70B-Instruct for all judge models.
 }\label{tab:evaluators}
\end{table*}


